Coherent Presentations of Monoidal Categories

Presentations of categories are a well-known algebraic tool to provide descriptions of categories by means of generators, for objects and morphisms, and relations on morphisms. We generalize here this notion, in order to consider situations where the objects are considered modulo an equivalence relation, which is described by equational generators. When those form a convergent (abstract) rewriting system on objects, there are three very natural constructions that can be used to define the category which is described by the presentation: one consists in turning equational generators into identities (i.e. considering a quotient category), one consists in formally adding inverses to equational generators (i.e. localizing the category), and one consists in restricting to objects which are normal forms. We show that, under suitable coherence conditions on the presentation, the three constructions coincide, thus generalizing celebrated results on presentations of groups, and we extend those conditions to presentations of monoidal categories.

==> dihedral.tex <==
\subsection{An example: the dihedral category $\Dcat_4$}
\label{sec:dihedral}
\PL{Je me demande si on ne devrait pas supprimer l’exemple dihédral (et renvoyer à la version conf), dans la mesure où nous avons un running exampple plus naturel dans ce papier.}
As an illustration of previous properties, we are going to study a presentation
of a category which is a variant of the dihedral group. Recall that the
\emph{dihedral group}~$D_n$ is the group of isometries of the plane preserving a
regular polygon with $n$ faces. This group is generated by a rotation~$r$ of
angle $2\pi/n$ and a reflection~$s$, and can be described as the free group over
the two generators $r$ and $s$ quotiented by the congruence generated by the
three relations $s^2=\id$, $r^n=\id$ and $rsr=s$.
%
We consider here a variant of this group: the category~$\Dcat_n$ of isometries
of the plane preserving a regular polygon with $n$ faces together with a
distinguished vertex (the category thus has $n$ objects). For instance, the
category $\Dcat_4$ is pictured on the left below, the distinguished vertex of
the square being pictured by a black triangle:
\begin{equation}
  \label{eq:dihedral}
  \vxym{
    \sq1\ar@/^1.5em/[rr]^{r_1} \ar@<.5ex>[rr]^{s_1} &&\sq2 \ar@<.5ex>[ll]^{s_2} \ar[d]^{r_2}\\
    \sq4 \ar[u]^{r_4} \ar@<.5ex>[rr]^{s_4} &&\sq3 \ar@/^1.5em/[ll]^{r_3} \ar@<.5ex>[ll]^{s_3}
  }
  \hspace{20ex}
  \vxym{
    \sq1 \ar@<-.5ex>[d]_{\ol{r_4}} \ar@/^1.5em/[rr]^{r_1} \ar@<.5ex>[rr]^{s_1} && \sq2 \ar@<.5ex>[ll]^{s_2} \ar[d]^{r_2} \ar@/^1.5em/[ll]^>>>>{\ol{r_1}}\\
    \sq4 \ar@<.5ex>[rr]^{s_4} \ar@<-.5ex>[u]_{r_4} \ar@/^1.5em/[rr]^>>>{\ol{r_3}} && \sq3 \ar@/^1.5em/[ll]^{r_3} \ar@<.5ex>[ll]^{s_3}
  }
\end{equation}
This category~$\Dcat_4$ admits a presentation~$P$ with 4 objects and 8
generating morphisms, as pictured on the left above, satisfying the 12
relations:
\begin{align*}
  r_{i+3}\circ r_{i+2}\circ r_{i+1}\circ r_i&=\id
  &
  s_{j+1}\circ s_j&=\id
  &
  r_j\circ s_{j+1}\circ r_j&=s_j
  \\
  &&
  s_j\circ s_{j+1}&=\id
  &
  r_{j+3}\circ s_{j+2}\circ r_{j+1}&=s_{j+1}
\end{align*}
for $i\in\set{1,\ldots,4}$ and $j\in\set{1,3}$, where the indices are to be
taken modulo $4$ so that they lie in $\set{1,\ldots,4}$.

% \[ s_2 \circ s_1 = \id, ~ s_1 \circ s_2 = \id, ~ s_4 \circ s_3 = \id, ~ s_3 \circ s_4 = \id \]
% \[r_4 \circ s_3 \circ r_2 =s_2 , ~r_2 \circ s_1 \circ r_4 = s_4,~ r_1 \circ s_2 \circ r_1 = s_1, ~ r_3 \circ s_4 \circ r_3 = s_3\]
% \[ r_4 \circ r_3 \circ r_2 \circ r_1 = \id, ~ r_1 \circ r_4 \circ r_3 \circ r_2 = \id, ~ r_2 \circ r_1 \circ r_4 \circ r_3 = \id , ~ r_3 \circ r_2 \circ r_1 \circ r_4 = \id \]

The methodology introduced earlier can be used to show that by quotienting
(\resp localizing) by $\Sigma=\set{r_2,r_4}$, we obtain a category which is
isomorphic (\resp equivalent) to~$\Dcat_2$: intuitively, ``forgetting'' about
those rotations quotients the square under symmetry \wrt an horizontal axis. We
thus consider the presentation modulo $(P,\tilde P_1)$ with $\tilde P_1=\Sigma$.
Unfortunately, this presentation does not satisfy the assumptions required to
apply our results; for instance, there is no residual of~$r_2$ after~$s_2$. It
is thus necessary to complete the presentation in order to have the confluence
properties (namely, the residuation and cylinder properties).
%
In rewriting theory, when a rewriting system is not confluent, one usually tries
to complete it (typically using a Knuth-Bendix completion algorithm) in order
for confluence to hold. Similarly, we can transform our presentation using a
series of Tietze transformations (Definition~\ref{def:tietze} and
Proposition~\ref{prop:tietze}) while preserving the same presented category, in
order to obtain another presentation of the same category which satisfies the
required assumptions.
%\SM{expliquer mieux: on complète pour pouvoir appliquer les théorèmes liés à la confluence}
% this is similar to the use of Knuth-Bendix completion in order to obtain a
% convergent rewriting system, see~\cite{guiraud2013homotopical} for details.

% A solution would be to add the generator $\ol r_4$ which would be an inverse
% of $r_4$ and localize and quotient by $\ol r_4$ rather than $r_4$. We are
% going to transform the presentation using Tietze-transformations in order to
% obtain that.

We first consider the presentation~$P'$ obtained from~$P$ by adding the new
generator $\ol r_4= r_3 \circ r_2 \circ r_1$ and its defining relation, as well
as the derivable relations $r_4 \circ \ol r_4 = \id$ and
$r_4 \circ \ol r_4 = \id$. We can now define~$r_2/s_2$ as $\ol r_4$, if we
consider $\ol r_4$ as an equational morphism. Fortunately, following lemma shows
that we can quotient, or localize, by $\ol r_4$ instead of~$r_4$, and we
therefore define $\tilde P'_1=\set{r_2,\ol r_4}$:

\begin{lemma}
  \label{lemma:quot-loc-inverse}
  Let~$P$ be a presentation of category such that there exist $f$ and $g$ in
  $P_1$ and two relations $f \circ g \ToT \id$ and $g \circ f \ToT \id$ in
  $P_2$. Let $\Sigma$ be a subset of $P_1$ not containing~$f$ nor~$g$. Then the
  quotients (\resp localizations) of $\pcat P$ by $\Sigma\uplus\set{f}$,
  $\Sigma\uplus\set{f,g}$, and $\Sigma\uplus\set{g}$ are isomorphic.
\end{lemma}
% \begin{proof}
%   The isomorphism of localizations follows from
%   Lemma~\ref{lem:presentation_loc_inverse} and the usual proof that a morphism
%   admits at most one inverse in a category. We now consider the case of
%   quotient:
%   %
%   we are going to show that the categories
%   $\pcat{P}_{f,g}=\pcat P/(\Sigma\uplus\set{f,g}$ and
%   $\pcat{P}_f=\pcat P/(\Sigma\uplus\set{f})$ are isomorphic. We write
%   $Q_{f,g} : \pcat{P} \to \pcat{P}_{f,g}$ and $Q_f : \pcat{P} \to \pcat{P}_f$
%   for the quotient functors. By the universal property of~$Q_f$, there exist a
%   unique $Q':\pcat{P}_f\to\pcat{P}_{f,g}$ such that $Q_{f,g} = Q' \circ Q_f$:
%   \[
%   \xymatrix{
%     \pcat{P} \ar[r]^{Q_f} \ar[d]_{Q_{f,g}} & \pcat{P}_f\ar@{..>}[dl]^{Q'}\\
%     \pcat{P}_{f,g}
%   }
%   \qquad\qquad
%   \xymatrix{
%     \pcat{P} \ar[r]^{Q_{f,g}} \ar[d]_{Q_f} & \pcat{P}_{f,g} \ar@{..>}[dl]^{F}\\
%     \pcat{P}_f
%   }
%   \qquad\qquad
%   \xymatrix{
%     \pcat{P} \ar[r]^{Q_f} \ar[d]_{Q_f} & \pcat{P}_f \ar@{..>}[dl]^{\Id} \ar[d]^{Q'}\\
%     \pcat{P}_f & \pcat{P}_{f,g} \ar[l]^{F}
%   }
%   \]
%   Moreover, since $Q_f (f) = \id$, we get that
%   $Q_f (g) = Q_f(g)\circ Q_f(f) = Q_f (g\circ f) = \id$ and therefore, by the
%   universal property of~$Q_{f,g}$, there exists a unique functor
%   $F:\pcat{P}_f\to\pcat{P}_{f,g}$ such that $Q_f =F\circ Q_{f,g}$. From these
%   equalities, we get that $Q_f =F\circ Q' \circ Q_f$ and that
%   $Q_{f,g} = Q' \circ F \circ Q_{f,g}$.
%   %
%   By universal property of~$Q_f$, the identity is the unique endofunctor of
%   $\pcat{P}_f$ such that $\id \circ Q_f = Q_f$, and therefore $F\circ Q'=\Id$.
%   Similarly, we have $Q' \circ I = \Id$, and therefore the categories
%   $\pcat{P}_f$ and $\pcat{P}_{f,g}$ are isomorphic.
% \end{proof}

\noindent
In this way, we have transformed the presentation~$(P,\tilde P_1)$ into a
presentation~$(P',\tilde P'_1)$ for which we can now define the residual
$r_2/s_2$. Similarly, in order for all the required residual to be defined, we
modify~$P'$ using Tietze transformations by adding generators
$\ol r_1 = r_4 \circ r_3 \circ r_2$ and $\ol r_3 = r_2 \circ r_1 \circ r_4$
and modifying the set of relations.
% First, we add the generators $\ol r_1 = r_4 \circ r_3 \circ r_2$ \FC{est-ce
% qu'on a besoin de l'introduire lui ? probablement pour op} and
% $\ol r_3 = r_2 \circ r_1 \circ r_4$ and their defining relations. We are able
% to deduce the relations $r_1 \circ \ol r_1 = \id$, $\ol r_1 \circ r_1 = \id$,
% $r_3 \circ \ol r_3 = \id$ and $\ol r_3 \circ r_3 = \id$ which we add to the
% presentation. We are now able to remove the relations
% $r_4 \circ r_3 \circ r_2 \circ r_1 = \id$ (deducible from
% $\ol r_4 = r_3 \circ r_2 \circ r_1$ and $r_4 \circ \ol r_4 = \id$) and
% $r_3 \circ r_2 \circ r_1 \circ r_4= \id$ (deducible from
% $\ol r_4 = r_3 \circ r_2 \circ r_1$ and $\ol r_4 \circ r_4 = \id$) from the
% presentation.  We can deduce the relations
% $r_2 \circ r_1 = \ol r_3 \circ \ol r_4$ and
% $r_3 \circ r_2 = \ol r_4 \circ \ol r_1$. We are able to remove the relations
% $r_2 \circ r_1 \circ r_4 \circ r_3 = \id$ (deducible from
% $r_2 \circ r_1 = \ol r_3 \circ \ol r_4$, $\ol r_4 \circ r_4 = \id$ and
% $\ol r_3 \circ r_3 = \id$) and $r_1 \circ r_4 \circ r_3 \circ r_2 = \id$
% (deducible from $r_3 \circ r_2 = \ol r_4 \circ \ol r_1$,
% $\ol r_1 \circ r_1 = \id$ and $\ol r_4 \circ r_4 = \id$). We can deduce the
% relations $s_3 \circ r_2 = \ol r_4 \circ s_2$ and
% $r_2 \circ s_1 = s_4 \circ \ol r_4$. We are able to remove the relations
% $ r_4 \circ s_3 \circ r_2 = s_2$ (deducible from
% $s_3 \circ r_2 = \ol r_4 \circ s_2$ and $r_4 \circ \ol r_4 = \id$) and
% $r_2 \circ s_1 \circ r_4 = s_4$ (deducible from
% $r_2 \circ s_1 = s_4 \circ \ol r_4$ and $\ol r_4 \circ r_4 = \id$). We are
% able to remove the relations $\ol r_4 = r_3 \circ r_2 \circ r_1$ (deducible
% from $\ol r_4 \circ \ol r_1 = r_3 \circ r_2$ and $\ol r_1 \circ r_1 = \id$),
% $\ol r_1 = r_4 \circ r_3 \circ r_2$ (deducible from
% $\ol r_4 \circ \ol r_1 = r_3 \circ r_2$ and $r_4 \circ \ol r_4 = \id$) and
% $\ol r_3 = r_2 \circ r_1 \circ r_4$ (deducible from
% $\ol r_3 \circ \ol r_4 = r_2 \circ r_1$ and $\ol r_4 \circ r_4 = \id$).
% Similarly to what was done before, we can replace the relation
% $s_3 = r_3 \circ s_4 \circ r_3$ by $\ol r_3 \circ s_3 \circ \ol r_3 = s_4$.
Finally, the presentation we end up with a presentation~$P''$ which has 11
morphism generators $r_i, s_i, \ol r_k$, as shown on the right
of~\eqref{eq:dihedral}, and 16 relations:
\begin{align*}
  s_{j+1}\circ s_j&=\id
  &
  r_1\circ s_2\circ r_1&=s_1
  &
  r_k \circ \ol r_k&= \id
  &
  r_2 \circ r_1&= \ol r_3 \circ \ol r_4
  &
  s_3 \circ r_2&= \ol r_4 \circ s_2
  \\
  s_j\circ s_{j+1}&=\id
  &
  \ol r_3 \circ s_3 \circ \ol r_3&=s_4
  &
  \ol r_k \circ r_k&= \id
  &
  r_3 \circ r_2&=\ol r_4 \circ \ol r_1
  &
  r_2 \circ s_1&= s_4 \circ \ol r_4
\end{align*}
% \[
% s_{j+1}\circ s_j=\id
% \quad
% s_j\circ s_{j+1}=\id
% \quad
% r_1\circ s_2\circ r_1=s_1
% \quad
% \ol r_3 \circ s_3 \circ \ol r_3 = s_4
% \quad
% r_k \circ \ol r_k = \id
% \quad
% \ol r_k \circ r_k = \id \]
% \[r_2 \circ r_1 = \ol r_3 \circ \ol r_4
% \quad
% r_3 \circ r_2 = \ol r_4 \circ \ol r_1
% \quad
% s_3 \circ r_2 = \ol r_4 \circ s_2
% \quad
% r_2 \circ s_1 = s_4 \circ \ol r_4
% \quad
% \]
for $i \in \set{1,\ldots,4}$, $j \in \set{1,3}$ and $k\in\set{1, 3, 4}$, which
is considered modulo $\tilde P''_1=\set{r_2,\ol r_4}$. This presentation modulo
is coherent. It satisfies convergence Assumption~\ref{apt:convergence}, and
residuals are defined by
\[
r_2 / s_2 = r_2 / \ol r_1 = \ol r_4
\quad
\ol r_4 / s_1 =\ol r_4 / r_1=r_2
\quad
s_1 / \ol r_4 = s_4
\quad
r_1 / \ol r_4 = \ol r_3
\quad
s_2 / r_2 = s_3
\quad
\ol r_1 / r_2 = r_3
\]
For termination Assumption~\ref{apt:1-termination}, we define $\omega_1$ as
equal to~$1$ on $s_1$, $s_2$, $\ol r_1$ and $r_1$ and $0$ on other morphism
generators. The cylinder Assumption~\ref{apt:cylinder} follows from considering
5 diagrams. For termination Assumption~\ref{apt:2-termination} we define
$\omega_2$ as $1$ on relation generators such that the only morphism generators
occurring in the source or the target are $r_1$, $\ol r_1$, $s_1$ or $s_2$, and
as $0$ otherwise. It can be checked similarly that
$(P''^\op, (\tilde P''_1)^\op)$ satisfies the assumptions.
%
% Does this presentation satisfy all our assumptions with $\ol r_4$ and $r_2$ as
% equational morphisms? We define the residuals $s_1 / \ol r_4 = s_4$,
% $\ol r_4 / s_1 = r_2$, $r_1 / \ol r_4 = \ol r_3$, $\ol r_4 / r_1 = r_2$,
% $s_2 / r_2 = s_3$, $r_2 / s_2 = \ol r_4$, $\ol r_1 / r_2 = r_3$ and
% $r_2 / \ol r_1 = \ol r_4$. This definition of residuation satisfies assumption
% \ref{apt:convergence}. The weight function which associates $1$ to $s_1$,
% $s_2$, $\ol r_1$ and $r_1$ and is zero on every other generator satisfies
% assumption \ref{apt:1-termination}. In order to check the cylinder property,
% there are cylinders to consider. We leave to the reader the computation of the
% cylinder property (assumption \ref{apt:cylinder}), it is satisfied. Besides,
% by constructing a weight function $w_2$ which associates $1$ to all relations
% between morphisms generated by $r_1, \ol r_1, s_1$ and $s_2$ and zero to all
% others, we get assumption \ref{apt:2-termination}. The opposite presentation
% is symmetric to this one, and thus satisfy Assumption~\ref{apt:op}.
%
Therefore $\nfcat{P''}{\set{r_2,\ol r_4}}$ is isomorphic to
$\pcat{P''}/\set{r_2,\ol r_4}$ by Theorem~\ref{thm:nf-quotient}, and equivalent
to $\loc{\pcat{P''}}{\set{r_2,\ol r_4}}$ by Theorem~\ref{thm:quotient-loc}, the
left-to-right part of the equivalence being an embedding by
Proposition~\ref{prop:loc_fidele}. An explicit (non-modulo) presentation for the
quotient can be obtained by Lemma~\ref{lemma:presentation-without-modulo}, and
this presentation is Tietze equivalent to the canonical presentation
of~$\Dcat_2$. We finally obtain the following result:

% Applying our result, we get that the localization of the category $\Dcat_4$ by
% $r_4$ and $r_2$ is equivalent to the quotient of $\Dcat_4$ by $r_4$ and $r_2$
% which is also the category of normal form \wrt $r_2$ and $\ol{r_4}$. As the
% quotient of $\Dcat_4$ by $r_4$ and $r_2$ is isomorphic to the quotient of
% $\Dcat_4$ by $r_4$, $\ol r_4$ and $r_2$ and given lemma
% \ref{lemma:presentation-without-modulo}, the quotient category
% $\Dcat_4 / \{ r_4, r_2 \}$ and the category of normal forms
% $\Nfcat{\Dcat_4}{\{\ol r_4, r_2 \}}$ is isomorphic to $\Dcat_2$.

% As illustration, we provide the following somewhat trivial example of a
% presentation of the monoid $\N\times\N$ (seen as a category) by a presentation
% modulo.
%
% Traditionaly, the monoid $\N \times \N$ is presented by the presentation
% $(\{ x \}, \{ a : x \to x, b : x \to x \}, \{ \gamma : b \circ a \To a \circ b
% \} )$,
% but it can also be presented by the presentation modulo $(P, \{c\})$ where
% \[P = (\{ x, y \}, \{ a, b : x \to x, c : x \to y, a', b' : y \to y \}, \{
% \gamma : b \circ a \To a \circ b, \gamma' : b' \circ a' \To a' \circ b' \}).\]
% This presentation modulo satisfies the assumptions that where previously made
% which means that $\pcat{P} [ \{ c \} ^{-1} ]$ is equivalent to
% $\pcat{P} _{ \{c\} }$ which is actually isomorphic to the category
% $\N \times \N$.

\begin{theorem}
  The category $\Dcat_2$ is isomorphic to the quotient $\Dcat_4/\set{r_2,r_4}$,
  embeds fully and faithfully into the category~$\Dcat_4$, and is equivalent to
  the localization~$\loc{\Dcat_4}{\set{r_2,r_4}}$.
\end{theorem}

\begin{remark}
  In this case, since~$r_2$ and~$r_4$ are already invertible in $\pcat{P}$, we
  moreover have $\loc{\Dcat_4}{\set{r_2,r_4}}\cong\Dcat_4$.
\end{remark}

\noindent
This illustrates the fact that, even though
Lemma~\ref{lem:presentation-without-modulo} indicates that presentations modulo
are not really necessary to present categories, the techniques developed here
around presentations modulo still lead to interesting results. Moreover, we will
see in next section that they generalize to presentations of monoidal
categories.

